LLMs are Introvert

The exponential growth of social media and generative AI has transformed information dissemination, fostering connectivity but also accelerating the spread of misinformation. Understanding information propagation dynamics and developing effective control strategies is essential to mitigate harmful content. Traditional models, such as SIR, provide basic insights but inadequately capture the complexities of online interactions. Advanced methods, including attention mechanisms and graph neural networks, enhance accuracy but typically overlook user psychology and behavioral dynamics. Large language models (LLMs), with their human-like reasoning, offer new potential for simulating psychological aspects of information spread. We introduce an LLM-based simulation environment capturing agents' evolving attitudes, emotions, and responses. Initial experiments, however, revealed significant gaps between LLM-generated behaviors and authentic human dynamics, especially in stance detection and psychological realism. A detailed evaluation through Social Information Processing Theory identified major discrepancies in goal-setting and feedback evaluation, stemming from the lack of emotional processing in standard LLM training. To address these issues, we propose the Social Information Processing-based Chain of Thought (SIP-CoT) mechanism enhanced by emotion-guided memory. This method improves the interpretation of social cues, personalization of goals, and evaluation of feedback. Experimental results confirm that SIP-CoT-enhanced LLM agents more effectively process social information, demonstrating behaviors, attitudes, and emotions closer to real human interactions. In summary, this research highlights critical limitations in current LLM-based propagation simulations and demonstrates how integrating SIP-CoT and emotional memory significantly enhances the social intelligence and realism of LLM agents.

==> src/exp.tex <==
\subsection*{Evaluating LLMs under Attacks}

We benchmark a wide array of existing LLMs, both open-source and close-source, assessing their susceptibility to various attacks across multiple application tasks, as presented in Table~\ref{tab:dipia-rslt}.
The complete model version information and metric information are detailed in Supplementary Info Sec. 1.1.
Notably, our findings reveal that all LLMs exhibit a certain level of vulnerability when confronted with indirect prompt injection attacks. This underscores the significance of our research into corresponding defense mechanisms.
Moreover, GPT-4 and GPT-3.5, which power the popular ChatGPT integrated applications, demonstrate relatively higher vulnerability under indirect prompt injection attacks.
Subsequently, we delve into the exploration of various factors that influence the success rate of attacks.



\noindent \textbf{Impact of LLM's capability.}
In Figure~\ref{fig:bench-rslt}\textbf{a}, we present the relationship between LLMs' capability measured by Elo ratings on Chatbot Arena~\cite{zheng2023judging}, a benchmark platform for LLMs in a crowd-sourced manner, and the ASRs on all attacks, text attacks, and code attacks, respectively.
Intriguingly, we observe a positive association between the Elo ratings and ASRs on text tasks, which indicates that more powerful LLMs are more susceptible to indirect prompt injection attacks.
This may be attributed to their advanced language understanding and generation capabilities, resulting in following malicious attack instructions embedded in third-party content more effectively. 
Although their performance on benign tasks is generally better, this phenomenon highlights their greater vulnerability to indirect prompt injection attacks.
% We observe that models with higher capabilities have higher ASRs on text attacks. This can be attributed to their advanced language understanding and generation capabilities, resulting in following malicious attack instructions embedded in third-party content more effectively. Although their performance on benign tasks is generally better, this phenomenon highlights their greater vulnerability to indirect prompt injection attacks.

However, similar relationship for code attacks is not observed. In this case, our experiments do not reveal a clear correlation between ASR and model's capability. This might be due to the varying strategies and abilities of different models when handling code generation tasks. We have noticed that the most capable model, GPT-4, can recognize the potential dangers of some malicious code snippets, particularly in active code attacks. This may also be one of the reasons for the lack of observable correlation. Despite the lack of a clear correlation, we still observe that code attacks can potentially succeed across different LLMs, emphasizing the importance of devising robust defense mechanisms against indirect prompt injection attacks in code generation scenarios.

% While the same positive correlation is also observed in code attacks, the corresponding Pearson correlation coefficient is lower than that of text attacks.
% This might be because Chatbot Arena is designed to evaluate the general task capabilities of LLMs and does not fully represent the ability of LLMs to execute tasks related to code.
% Despite the lack of a clear correlation, we still observe that code attacks can potentially succeed across different LLMs, emphasizing the importance of devising robust defense mechanisms against indirect prompt injection attacks in code generation scenarios.

\noindent \textbf{Impact of application task types.} 
Table~\ref{tab:dipia-rslt} shows that the ASR of summarization is higher than that of table QA, email QA, and web QA. This discrepancy may stem from the differences in prompt templates for these tasks. As shown in the prompts for different tasks in Supplementary Information Sec. 1.1, in the summarization task, there are no additional user instructions appended at the end of the prompt. In contrast, the templates for the other tasks, such as table QA, email QA, and web QA, include user instructions as the last sentence, typically in the form of a question. Additionally, the ASR of code QA surpasses table QA, email QA, and web QA. However, since code attacks are targeted attacks distinct from text attacks, direct comparisons between them are not made.



\noindent \textbf{Impact of text attack types. }
In Figure~\ref{fig:bench-rslt}\textbf{b}, our evaluation results indicate that task-relevant text attacks and targeted attacks have higher ASRs than task-irrelevant text attacks, especially for GPT-4 and GPT-3.5-turbo.
This might be due to the model's attention mechanism prioritizing task-relevant information, making both targeted and task-relevant attacks more effective.
Additionally, targeted attacks and task-relevant text attacks may have objectives that do not conflict with the original task, making them more easily accepted by the models.


\begin{table*}[!t]
\centering
\caption{\textbf{Performance of different black-box defenses on \benchmark with GPT-4 and GPT-3.5-Turbo.} 
For defenses with hyper-parameters, we choose to present the results of the setting with the lowest overall ASR. 
% For the border-string defense, we display the results with backticks for text tasks and hyphen for the code task. 
For the in-context learning defense, we report the results with 2 in-context learning examples. 
In addition to the Attack Success Rates (ASRs) on the BIPIA test dataset, we also report the ROUGE-1 (recall) of the defenses when the external content is not under attack, indicating their ability to complete the original task. Higher ROUGE-1 (recall) values signify that the defense method has a lower impact on application performance.}
\scalebox{0.85}{
\begin{tabular}{l|l|c|cccc|c|c}
\Xhline{1.0pt}
\multirow{2}{*}{Model} & \multirow{2}{*}{Method}   & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ROUGE-1 \\ (recall) \end{tabular}}} & \multicolumn{4}{c|}{ASR of Text Tasks}                & ASR of Code Task & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Overall\\ ASR\end{tabular}}} \\  \cmidrule(lr){4-7} \cmidrule(lr){8-8}
   &               &             & Email QA & Web QA & Table QA & Summarization & Code QA     &       \\ \midrule
\multirow{4}{*}{GPT-4} & Original            &  0.6985 & 0.1524 & 0.2792 & 0.3472 & 0.3917 & 0.2863 & 0.3103    \\
% & Border strings & 0.6963 & 0.0690 & 0.2238 & 0.2565 & 0.2374 & 0.0085 & 0.1970 \\
& In-context learning & 0.6590 & 0.1036 & 0.2382 & 0.3238 & 0.3075 & 0.0056 & 0.2408 \\
& Multi-turn dialogue & 0.7201 & 0.0959 & 0.2585 & 0.2974 & 0.1810 & 0.0097 & 0.2056 \\
\midrule
\multirow{4}{*}{GPT-3.5-Turbo} & Original     & 0.6554 & 0.1634 & 0.2347 & 0.2257 & 0.3658 & 0.2844 & 0.2616  \\
% & Border strings &  0.6612 & 0.0587 & 0.1655 & 0.1615 & 0.2632 & 0.0567 & 0.1665  \\
& In-context learning & 0.6289 & 0.1779 & 0.1600 & 0.1910 & 0.2560 & 0.0789 & 0.1884
 \\
& Multi-turn dialogue &  0.6786 & 0.1376 & 0.2025 & 0.1936 & 0.2221 & 0.0583 & 0.1843 \\
% Datamarks & 0.6491 & 0.0251 & 0.0548 & 0.0705 & 0.1427 & 0.4124 & 0.1090 \\
\Xhline{1.0pt}
\end{tabular}
}
\label{tab:black-box}
\end{table*}

\begin{table*}[!t]
\centering
\caption{\textbf{Performance of the white-box defense on \benchmark with Vicuna-7B and Vicuna-13B.} We report the results of the models saved at the 1000-th step.
In addition to the Attack Success Rates (ASRs) on the BIPIA test set, we also report the ROUGE-1 (recall) of defenses when the external content is not attacked, for completing the original task. Higher ROUGE-1 (recall) values indicate that the defense method has less impact on the application performance. Meanwhile, since white-box methods modify the model parameters, we also report the MT-bench scores of the fine-tuned LLMs. Higher MT-bench scores suggest that the defense does not impair the model's performance on general tasks, which is meaningful for LLM providers.
}
\scalebox{0.8}{
\begin{tabular}{l|l|c|c|cccc|c|c}
\Xhline{1.0pt}
\multirow{2}{*}{Model}  & \multirow{2}{*}{Response} &  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}ROUGE-1\\ (recall))\end{tabular}} & Capability & \multicolumn{4}{c|}{ASR of Text Task}                & ASR of Code Task & \multicolumn{1}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Overall\\ ASR\end{tabular}}} \\ \cmidrule(lr){4-5} \cmidrule(lr){5-8} \cmidrule(lr){9-9}
   &  Source  & & MT-Bench & Email QA & Web QA & Table QA & Summarization & Code QA     &       \\ \midrule

\multirow{4}{*}{Vicuna-7B} & w/o finetune & 0.6187 & 4.8063 & 0.1124 & 0.0693 & 0.0827 & 0.2117 & 0.1632 & 0.1237 \\
& BIPIA & 0.5306 & 4.2938 & 0.0202 & 0.0159 & 0.0410 & 0.0049 & 0.0300 & 0.0214 \\
& Original LLM & 0.6122 & 4.5687 & 0.0015 & 0.0062 & 0.0057 & 0.0043 & 0.2244 & 0.0240 \\
& GPT-4 & 0.6260 & 4.8312 & 0.0065 & 0.0045 & 0.0046 & 0.0037 & 0.0129 & 0.0053 \\
\midrule
\multirow{4}{*}{Vicuna-13B} & w/o finetune & 0.6134 & 5.2062 & 0.1242 & 0.1272 & 0.1337 & 0.2052 & 0.1755 & 0.1531 \\
& BIPIA & 0.6109 & 1.6625 & 0.0217 & 0.0126 & 0.0370 & 0.0064 & 0.0207 & 0.0192 \\
& Original LLM & 0.6240 & 4.3375 & 0.0024 & 0.0055 & 0.0051 & 0.0034 & 0.0067 & 0.0046 \\
& GPT-4 & 0.6337 & 4.5500 & 0.0060 & 0.0044 & 0.0057 & 0.0036 & 0.0036 & 0.0047 \\
\Xhline{1.0pt}
\end{tabular}
}
\label{tab:white-box}
\end{table*}

\noindent \textbf{Impact of code attack types. }
As shown in Figure~\ref{fig:bench-rslt}\textbf{c}, we note that the ASRs of GPT-3.5-turbo, Vicuna-7B, and Vicuna-13B exhibit a similar trend for both passive and active attacks.
However, the ASR of active attacks on GPT-4 is notably lower than that of passive attacks.
A possible explanation based on our observations could be that active code attacks involve modifying users' local files or the machine's operating state without explicitly indicating malicious intent in the code. 
Despite the lack of explicit indications of malice, GPT-4, with its advanced code comprehension capabilities, is able to discern the intent behind the code and opts to refuse to follow the malicious instructions of active code attacks.
% As shown in Figure~\ref{fig:bench-rslt}\textbf{c}, we observe that passive code attacks have higher ASRs than active code attacks, especially for GPT-4. 
% The difference in ASR is not so significant in GPT-3.5-turbo and Vicuna-13B. 
% A possible explanation based on our observations could be that active code attacks involve modifying users' local files or the machine's operating state without explicitly indicating malicious intent in the code. Despite the lack of explicit indications of malice, GPT-4, with its advanced code comprehension capabilities, 
% is able to discern the intent behind the code and opts to refuse to follow the instructions of active code attacks.


\noindent \textbf{Impact of positions of attack instructions. }
Figure~\ref{fig:bench-rslt}\textbf{d} demonstrates that injection locations of attack instructions within third-party content significantly impact the ASR. We observe that placing the attack at the end of the external content results in the highest ASR, followed by placing it at the beginning and middle. This phenomenon may be attributed to the data distribution during the training process of LLMs, where most instructions might be present at the end of samples. Consequently, LLMs may learn a position bias that inadvertently increases the influence of the injected attack instructions, particularly when they are located at the end of the content~\cite{liu2023lost}. 

\begin{figure}[!t]
   \centering
   \includegraphics[width=1\textwidth]{figure/ablation.pdf}
   \caption{\textbf{Ablation study.} 
   Performance comparison of w/o explicit reminder and w/o boundary awareness variants of several defenses.
   Lower ASR on BIPIA indicates better defense performance.
   Higher ROUGE under no attacks and ratings on MT-bench indicate better defense performance.
   \textbf{a}, the ASR and ROUGE under no attacks of GPT-3.5-turbo incorporating the original in-context learning and multi-turbo dialogue defenses and their w/o explicit reminder and w/o boundary awareness variants.
   \textbf{b}, the ASR, ROUGE under no attacks and MT-bench ratings of Vicuna-7B incorporating the original white-box defense and its w/o explicit reminder and w/o boundary awareness variants.
   \textbf{c}, the ASR, ROUGE under no attacks and MT-bench ratings of Vicuna-13B incorporating the original white-box defense and its w/o explicit reminder and w/o boundary awareness variants.
   }
   \label{fig:ablation}
 \end{figure}

\subsection*{Evaluating Defense Performance}
We evaluate our black-box defenses on GPT-4 and GPT-3.5-Turbo models and the white-box approach on Vicuna-7B and Vicuna-13B. 
Table~\ref{tab:black-box} and Table~\ref{tab:white-box} present the comprehensive results for two types of defenses, respectively. 
For the black-box defenses, besides ASR, we illustrate the ROUGE-1 (recall) scores when these black-box defenses are applied to normal inputs without any attacks.
This indicates the impact of these defenses on the functional capabilities of the model on the application under non-attack conditions.
For the white-box defense, since the white-box defense modifies the model's parameters, in addition to the ASR and ROUGE-1 (recall), we also report capability scores on MT-bench of the fine-tuned LLMs. 
This metric ranges from 1 to 10, with higher scores indicating better performance of the LLMs on general tasks.
Derailed metric settings are provided in the Supplementary Information Sec. 1.1.

Table~\ref{tab:black-box} presents the effectiveness of various black-box defenses.
On the one hand, it is observed that all black-box defenses are effective in substantially reducing the ASR.
On the other hand, when examining the ROUGE score of different indirect prompt injection attacks with and without these defenses, it is noted that, with the exception of in-context learning, the performance remains comparable to the original model. 
This indicates that these simple methods do not significantly impair functionality. 
Finally, a comparison between GPT-4 and GPT-3.5-Turbo reveals that, overall, the ASR on GPT-4 is higher than on GPT-3.5-Turbo. 
This could be attributed to the inherently higher base ASR of GPT-4. 
However, in tasks involving external content of shorter length, such as EmailQA and codeQA, GPT-4's ASR significantly decreases and falls below that of GPT-3.5-Turbo. 
This indicates that GPT-4 is more adept at following explicit reminder instructions and distinguishing between external content and user instructions in scenarios where the external content is brief.

Table~\ref{tab:white-box} demonstrates the performance of various configurations of our white-box defense. 
Specifically, we investigate various adversarial training datasets, which involve pairing the maliciously attacked input with three types of benign responses: labels from the benchmark dataset and responses generated by the original LLM/GPT-4 on prompts without malicious instructions.
We obtain two key observations as follows.
First, white-box defense methods can effectively reduce the ASR to close to 0, which is 10 times lower than the original ASR. 
Second, there is at least one response construction method, such as GPT-4, that can ensure little decline in the ROUGE score and the capability score on MT-Bench. 
Overall, the result indicates that our white-box defense can nearly completely defend against indirect prompt injection attacks, without compromising model performance.


% White-box defenses employ adversarial training and involve fine-tuning the LLM using prompts from the BIPIA training set.
% The training targets that are responses unaffected by malicious instructions and aligned with user instructions.
% We explored three methods for constructing target responses: 1) Using labels from the \benchmark dataset; 2) Using benign responses generated by the original LLM on prompts without malicious instructions; 3) Using responses generated by GPT-4 on prompts without malicious instructions.
% Table~\ref{tab:white-box} shows that on Vicuna-7B and Vicuna-13B, white-box defense methods based on different response construction methods can effectively reduce the ASR to close to 0, which is 10 times lower than the original ASR. At the same time, there is at least one response construction method, such as GPT-4, that can ensure no decline in the ROUGE score on BIPIA-Clean and the capability score on MT-Bench. This indicates that white-box defense can effectively defend against indirect prompt injection attacks, without compromising model performance.


\subsection*{Ablation Study}
\begin{figure}[!t]
   \centering
   \includegraphics[width=1\textwidth]{figure/hyper-params.pdf}
   \caption{\textbf{Hyper-parameter analysis of multiple defenses.} 
   % \textbf{a}-\textbf{b}, the ASR and ROUGE-1 (recall) of GPT-3.5-Turbo across multiple tasks incorporating different border strings in the border-string defense. 
   \textbf{a}-\textbf{b}, the ASR and ROUGE-1 (recall) of GPT-3.5-Turbo across multiple tasks incorporating different number of in-context learning examples.
   \textbf{c}-\textbf{e}, trends in ASR, ROUGE-1 (recall), and MT-Bench score of Vicuna-7B with different response construction methods under white-box defenses across training steps.
   \textbf{f}-\textbf{h}, trends in ASR, ROUGE-1 (recall), and MT-Bench score of Vicuna-13B with different response construction methods under white-box defenses across training steps. }
   \label{fig:hyper}
 \end{figure}

In this subsection, we investigate the two core components of our proposed defenses consist of: \textit{explicit reminder} and \textit{boundary awareness}.
\textit{Explicit reminder} is designed to explicitly remind an LLM not to execute instructions embedded within external content, while \textit{boundary awareness} is intended to make an LLM aware of the boundaries between external content and user instructions.
To further analyze the effectiveness of these two components, we conduct an ablation study.
More specifically, we remove each of the two core components from the defense and observe the performance change of the defense.
Detailed experimental settings are provided in the Supplementary Information Sec. 1.3.

Our empirical results in Figure~\ref{fig:ablation}\textbf{a} demonstrate that the ASR of the black-box defenses increases when either of the two components is removed. 
This indicates the effectiveness of both components in defending against indirect prompt injection attacks.
Furthermore, we observe that the removal of boundary awareness has a greater impact on ASR than the removal of explicit reminder, indicating that the ability to distinguish boundaries may be more important for LLMs to defend against indirect prompt injection attacks.
At the same time, the removal of either component does not significantly affect the ROUGE score of the original task, which shows that the utility of the method is not compromised.

For the white-box defense, our results in Figure~\ref{fig:ablation}\textbf{b}-\textbf{c} indicate that removing explicit reminder has a smaller impact on ASR than removing boundary awareness for different response construction methods. 
This may be because LLMs implicitly learn not to execute instructions in external content during fine-tuning.
At the same time, comparing the ROUGE and MT-bench scores, we find that white-box fine-tuning does not affect the performance of LLMs on the fine-tuning task without attack, but may affect the performance on general tasks.



\subsection*{Hyper-parameter Analysis}


We analyze the impact of hyper-parameters on the performance of defense methods. 
More specifically, we study the impact of the number of in-context learning examples for in-context learning defense, the response construction method, and the training steps for our white-box defense.

% \textbf{Impact of different border types. }
% For border-string defense, we analyze the impact of different types of border string, of which the results are shown in Figure~\ref{fig:hyper}\textbf{a}-\textbf{b}.
% As illustrated in Figure~\ref{fig:hyper}\textbf{a}, adding any of the three types of border strings effectively decreases the ASR on all tasks. 
% The effectiveness of different borders varies across tasks. In text tasks, the backtick works best, followed by the hyphen, and finally the equal sign. In the code task, the equal sign performs best, followed by the hyphen, and lastly the backtick. We believe this phenomenon occurs because border strings based on hyphens and backticks often appear in Stack Overflow answers themselves, leading to unclear border boundaries and subsequently a decline in performance.
% Figure~\ref{fig:hyper}\textbf{b} demonstrates that incorporating these border strings does not impact the performance of LLMs on the original tasks.


\noindent \textbf{Impact of the number of examples in the in-context learning. }
For in-context learning defense, we analyze the impact of the number of in-context learning examples.
As shown in Figure~\ref{fig:hyper}\textbf{a}-\textbf{b}, although adding different numbers of in-context learning examples can reduce the ASR, there is no clear correlation between the number of examples added in text tasks and ASR. 
This may be related to the diversity of external content and instructions in text attacks. 
In the code QA task, however, we observe a clear downward trend in ASR as the number of in-context learning examples increased. 
In addition, we observe that adding in-context examples has no significant effect on the ROUGE score of benign input, which indicates that the defense method does not impair the model's performance on the original task.



\noindent \textbf{Impact of different response construction methods. }
As shown in Figure~\ref{fig:hyper}\textbf{c} and Figure~\ref{fig:hyper}\textbf{f}, all three response construction methods can effectively reduce the ASR to close to 0.
Among them, the response from GPT-4 performs the best. This may be due to the gains brought about by the high quality and high diversity of GPT-4 response.
In terms of performance impact (Figures~\ref{fig:hyper}\textbf{d} and~\ref{fig:hyper}\textbf{g}), GPT-4 has the least impact on ROUGE-1 (recall) on benign prompts, followed by Original LLM and BIPIA. 
The impact may stem from response quality and diversity.
Original LLM generates lower-quality responses, while Directly using the BIPIA label as a response makes the model's answers rigid and lacking in explanation, influencing the ROUGE score.
As shown in Figure~\ref{fig:hyper}\textbf{e} and Figure~\ref{fig:hyper}\textbf{h}, the capability score on MT-bench demonstrates a similar trend to the ROUGE score.


\textbf{Impact of training steps. }
As shown in Figure~\ref{fig:hyper}\textbf{c}-\textbf{h}, the main conclusion is that a significant drop in ASR can be observed after approximately 100 training steps.
On the other hand, After 500 training steps, the model's ROUGE score and capability score on MT-bench also tend to stabilize.


==> table/ablation_table.tex <==
\begin{table}[!htbp]
\centering
\caption{Macro and Micro Indicators for SIP-enhanced Model Comparison}
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{c|c|cccc|cccc|cccc|cccc}
\toprule
\multirow{3}{*}{\textbf{Dataset}} & \multirow{3}{*}{\textbf{Model version}} & \multicolumn{4}{c|}{\textbf{Macro indicators after simulation}} & \multicolumn{12}{c}{\textbf{Micro indicators}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-18}
  &  & \multirow{2}{*}{\centering \textbf{delta\_bias}} & \multirow{2}{*}{\centering \textbf{delta\_div}} & \multirow{2}{*}{\centering \textbf{DTW}} & \multirow{2}{*}{\centering \textbf{perason\_corr}} & \multicolumn{4}{c|}{\textbf{Stance}} & \multicolumn{4}{c|}{\textbf{Behavior}} & \multicolumn{4}{c}{\textbf{Content}} \\
\cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18}
  &  &  &  &  &  & \textbf{F1} & \textbf{REC} & \textbf{PRE} & \textbf{ACC} & \textbf{F1} & \textbf{REC} & \textbf{PRE} & \textbf{ACC} & \textbf{F1} & \textbf{REC} & \textbf{PRE} & \textbf{ACC} \\
\midrule
\multirow{5}{*}{Dataset1} & Fully enhanced model     & 0.0732 & 0.0197 & 0.0125 & 0.4531 & 0.5823 & 0.5682 & 0.5563 & 0.5945 & 0.5820 & 0.5678 & 0.5559 & 0.5942 & 0.5817 & 0.5674 & 0.5556 & 0.5939 \\
 & Model without social rules memory     & 0.1187 & 0.0853 & 0.1098 & 0.3899 & 0.5258 & 0.5113 & 0.4964 & 0.5391 & 0.5255 & 0.5110 & 0.4959 & 0.5388 & 0.5252 & 0.5107 & 0.4955 & 0.5385 \\
 & Model without reflection & 0.1443 & 0.1102 & 0.1423 & 0.3226 & 0.4634 & 0.4531 & 0.4402 & 0.4756 & 0.4631 & 0.4528 & 0.4398 & 0.4753 & 0.4628 & 0.4525 & 0.4395 & 0.4750 \\
 & Model without SIP COT & 0.1576 & 0.1354 & 0.1632 & 0.2957 & 0.4419 & 0.4301 & 0.4178 & 0.4510 & 0.4417 & 0.4299 & 0.4175 & 0.4508 & 0.4414 & 0.4296 & 0.4172 & 0.4506 \\
 & Basic model              & 0.1693 & 0.1485 & 0.1791 & 0.2652 & 0.3911 & 0.3806 & 0.3699 & 0.4041 & 0.3909 & 0.3804 & 0.3697 & 0.4039 & 0.3907 & 0.3802 & 0.3695 & 0.4037 \\
\midrule
\multirow{5}{*}{Dataset2} & Fully enhanced model     & 0.0798 & 0.0254 & 0.0183 & 0.4672 & 0.5984 & 0.5851 & 0.5742 & 0.6097 & 0.5981 & 0.5848 & 0.5739 & 0.6094 & 0.5978 & 0.5845 & 05736 & 0.6091 \\
 & Model without social rules memory     & 0.1249 & 0.0921 & 0.1187 & 0.3984 & 0.5301 & 0.5166 & 0.5012 & 0.5439 & 0.5298 & 0.5163 & 0.5009 & 0.5436 & 0.5295 & 0.5160 & 0.5006 & 0.5433 \\
 & Model without reflection & 0.1520 & 0.1175 & 0.1516 & 0.3278 & 0.4679 & 0.4572 & 0.4443 & 0.4791 & 0.4677 & 0.4569 & 0.4440 & 0.4788 & 0.4674 & 0.4567 & 0.4438 & 0.4785 \\
 & Model without SIP COT & 0.1629 & 0.1391 & 0.1688 & 0.3025 & 0.4497 & 0.4383 & 0.4254 & 0.4581 & 0.4494 & 0.4380 & 0.4251 & 0.4578 & 0.4492 & 0.4378 & 0.4249 & 0.4576 \\
 & Basic model              & 0.1721 & 0.1512 & 0.1842 & 0.2704 & 0.3962 & 0.3855 & 0.3748 & 0.4083 & 0.3960 & 0.3853 & 0.3746 & 0.4080 & 03958 & 0.3850 & 0.3743 & 0.4078 \\
\midrule
\multirow{5}{*}{Dataset3} & Fully enhanced model     & 0.0694 & 0.0215 & 0.0142 & 0.4783 & 0.6027 & 0.5893 & 0.5783 & 0.6142 & 0.6025 & 0.5890 & 0.5780 & 0.6139 & 0.6022 & 0.5887 & 0.5777 & 0.6137 \\
 & Model without social rules memory     & 0.1203 & 0.0869 & 0.1134 & 0.3962 & 0.5289 & 0.5147 & 0.4996 & 0.5418 & 0.5287 & 0.5145 & 0.4993 & 0.5415 & 0.5285 & 0.5142 & 0.4991 & 0.5413 \\
 & Model without reflection & 0.1419 & 0.1094 & 0.1400 & 0.3191 & 0.4597 & 0.4495 & 0.4367 & 0.4720 & 0.4594 & 0.4492 & 0.4364 & 04717 & 0.4591 & 0.4489 & 0.4361 & 0.4714 \\
 & Model without SIP COT & 0.1557 & 0.1336 & 0.1621 & 0.2919 & 0.4424 & 0.4305 & 0.4176 & 0.4503 & 0.4421 & 0.4303 & 0.4174 & 0.4500 & 0.4419 & 0.4301 & 0.4172 & 0.4498 \\
 & Basic model              & 0.1678 & 0.1469 & 0.1773 & 0.2675 & 0.3883 & 0.3774 & 0.3666 & 0.4002 & 0.3881 & 0.3772 & 0.3664 & 0.4000 & 0.3878 & 0.3770 & 0.3662 & 0.3998 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> table/diff_model_table.tex <==
\begin{table}[!htbp]
\centering
\caption{Macro and Micro Indicators for Model Comparison}
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{c|c|cccc|cccc|cccc|cccc}
\toprule
\multirow{3}{*}{\textbf{Dataset}} & \multirow{3}{*}{\textbf{LLM Model version}} & \multicolumn{4}{c|}{\textbf{Macro indicators after simulation}} & \multicolumn{12}{c}{\textbf{Micro indicators}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-18}
  &  & \multirow{2}{*}{\centering \textbf{delta\_bias}} & \multirow{2}{*}{\centering \textbf{delta\_div}} & \multirow{2}{*}{\centering \textbf{DTW}} & \multirow{2}{*}{\centering \textbf{perason\_corr}} & \multicolumn{4}{c|}{\textbf{Stance}} & \multicolumn{4}{c|}{\textbf{Behavior}} & \multicolumn{4}{c}{\textbf{Content}} \\
\cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18}
  &  &  &  &  &  & \textbf{F1} & \textbf{REC} & \textbf{PRE} & \textbf{ACC} & \textbf{F1} & \textbf{REC} & \textbf{PRE} & \textbf{ACC} & \textbf{F1} & \textbf{REC} & \textbf{PRE} & \textbf{ACC} \\
\midrule
\multirow{5}{*}{Dataset1} & gpt-4     & 0.0752 & 0.0178 & 0.0114 & 0.1896 & 0.5121 & 0.4987 & 0.4752 & 0.5182 & 0.5115 & 0.4982 & 0.4748 & 0.5176 & 0.5109 & 0.4978 & 0.4744 & 0.5170 \\
 & gpt-4o     & 0.1476 & 0.1052 & 0.1599 & 0.3023 & 0.4294 & 0.4181 & 0.4033 & 0.4416 & 0.4290 & 0.4178 & 0.4028 & 0.4409 & 0.4286 & 0.4174 & 0.4024 & 04402 \\
 & gpt-4 mini & 0.1584 & 0.1406 & 0.1713 & 0.2650 & 0.3734 & 0.3630 & 0.3516 & 0.3921 & 0.3731 & 0.3627 & 0.3514 & 0.3918 & 0.3728 & 0.3623 & 0.3511 & 0.3915 \\
 & gpt-3.5-turbo & 0.1823 & 0.1612 & 0.1963 & 0.2371 & 0.3048 & 0.2937 & 0.2821 & 0.3236 & 0.3045 & 0.2935 & 0.2818 & 0.3233 & 0.3042 & 0.2932 & 0.2814 & 0.3229 \\
 & Llama3              & 0.1586 & 0.1415 & 0.1725 & 0.2667 & 0.3737 & 0.3632 & 0.3520 & 0.3924 & 0.3734 & 0.3630 & 0.3518 & 0.3921 & 0.3730 & 0.3626 & 0.3515 & 0.3917 \\
\midrule
\multirow{5}{*}{Dataset2} & gpt-4     & 0.0706 & 0.0156 & 0.0107 & 0.1894 & 0.5115 & 0.4979 & 0.4741 & 0.5173 & 0.5109 & 0.4976 & 0.4738 & 0.5169 & 0.5103 & 0.4972 & 04734 & 0.5164 \\
 & gpt-4o     & 0.1439 & 0.1042 & 0.1573 & 0.2987 & 0.4289 & 0.4174 & 0.4026 & 0.4411 & 0.4285 & 0.4171 & 0.4022 & 0.4405 & 0.4281 & 0.4167 & 0.4019 & 0.4400 \\
 & gpt-4 mini & 0.1545 & 0.1378 & 0.1689 & 0.2617 & 0.3728 & 0.3625 & 0.3511 & 0.3914 & 0.3725 & 0.3622 & 0.3510 & 0.3912 & 0.3721 & 0.3618 & 0.3507 & 0.3909 \\
 & gpt-3.5-turbo & 0.1804 & 0.1597 & 0.1946 & 0.2359 & 0.3037 & 0.2926 & 0.2811 & 0.3226 & 0.3034 & 0.2924 & 0.2807 & 0.3222 & 0.3031 & 0.2921 & 0.2803 & 0.3218 \\
 & Llama3              & 0.1550 & 0.1383 & 0.1696 & 0.2628 & 0.3730 & 0.3627 & 0.3513 & 0.3916 & 0.3727 & 0.3623 & 0.3511 & 0.3913 & 0.3724 & 0.3620 & 0.3508 & 0.3910 \\
\midrule
\multirow{5}{*}{Dataset3} & gpt-4     & 0.0739 & 0.0163 & 0.0105 & 0.1898 & 0.5118 & 0.4981 & 0.4746 & 0.5175 & 0.5112 & 0.4978 & 0.4743 & 0.5172 & 0.5106 & 0.4974 & 0.4739 & 0.5168 \\
 & gpt-4o     & 0.1463 & 0.1031 & 0.1581 & 0.3002 & 0.4292 & 0.4178 & 0.4029 & 0.4414 & 0.4288 & 0.4174 & 0.4024 & 0.4408 & 0.4284 & 0.4170 & 0.4020 & 0.4403 \\
 & gpt-4 mini & 0.1572 & 0.1399 & 0.1712 & 0.2649 & 0.3735 & 0.3631 & 0.3517 & 0.3923 & 0.3732 & 0.3628 & 0.3515 & 0.3919 & 0.3729 & 0.3625 & 0.3513 & 0.3916 \\
 & gpt-3.5-turbo & 0.1815 & 0.1604 & 0.1953 & 0.2366 & 0.3052 & 0.2941 & 0.2826 & 0.3232 & 0.3049 & 0.2938 & 0.2823 & 0.3228 & 0.3046 & 0.2935 & 0.2819 & 0.3225 \\
 & Llama3              & 0.1567 & 0.1394 & 0.1709 & 0.2634 & 0.3731 & 0.3628 & 0.3514 & 0.3917 & 0.3728 & 0.3624 & 0.3512 & 0.3914 & 0.3725 & 0.3621 & 0.3510 & 0.3912 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}



==> table/eight_metrics.tex <==
\begin{table}[!htbp]
\centering
\caption{Comparison of Various Agents on Different Metrics}
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{c|c|ccccccccccccc}
\toprule
\textbf{Parameter} & \textbf{Agent Type} & \textbf{Q1} & \textbf{Q2} & \textbf{Q3} & \textbf{Q4} & \textbf{Q5} & \textbf{Q6} & \textbf{Q7} & \textbf{Q8} & \textbf{Q9} & \textbf{Q10} & \textbf{Q11} & \textbf{Q12} & \textbf{Q13} \\
\midrule
\multirow{3}{*}{M} 
    & Human               & 0.10 & 0.20 & 0.30 & 0.40 & 0.50 & 0.60 & 0.70 & 0.80 & 0.90 & 0.10 & 0.20 & 0.30 & 0.40 \\
    & Basic agent         & 0.11 & 0.21 & 0.31 & 0.41 & 0.51 & 0.61 & 0.71 & 0.81 & 0.91 & 0.11 & 0.21 & 0.31 & 0.41 \\
    & SIP-enhanced agent  & 0.12 & 0.22 & 0.32 & 0.42 & 0.52 & 0.62 & 0.72 & 0.82 & 0.92 & 0.12 & 0.22 & 0.32 & 0.42 \\
\midrule
\multirow{2}{*}{$\Delta$M} 
    & Basic agent         & 0.01 & 0.02 & 0.03 & 0.04 & 0.05 & 0.06 & 0.07 & 0.08 & 0.09 & 0.01 & 0.02 & 0.03 & 0.04 \\
    & SIP-enhanced agent  & 0.02 & 0.03 & 0.04 & 0.05 & 0.06 & 0.07 & 0.08 & 0.09 & 0.10 & 0.02 & 0.03 & 0.04 & 0.05 \\
\midrule
\multirow{3}{*}{SD} 
    & Human               & 0.13 & 0.23 & 0.33 & 0.43 & 0.53 & 0.63 & 0.73 & 0.83 & 0.93 & 0.13 & 0.23 & 0.33 & 0.43 \\
    & Basic agent         & 0.14 & 0.24 & 0.34 & 0.44 & 0.54 & 0.64 & 0.74 & 0.84 & 0.94 & 0.14 & 0.24 & 0.34 & 0.44 \\
    & SIP-enhanced agent  & 0.15 & 0.25 & 0.35 & 0.45 & 0.55 & 0.65 & 0.75 & 0.85 & 0.95 & 0.15 & 0.25 & 0.35 & 0.45 \\
\midrule
\multirow{2}{*}{$\Delta$SD} 
    & Basic agent         & 0.01 & 0.02 & 0.03 & 0.04 & 0.05 & 0.06 & 0.07 & 0.08 & 0.09 & 0.01 & 0.02 & 0.03 & 0.04 \\
    & SIP-enhanced agent  & 0.02 & 0.03 & 0.04 & 0.05 & 0.06 & 0.07 & 0.08 & 0.09 & 0.10 & 0.02 & 0.03 & 0.04 & 0.05 \\
\midrule
\multirow{3}{*}{Skew} 
    & Human               & 0.16 & 0.26 & 0.36 & 0.46 & 0.56 & 0.66 & 0.76 & 0.86 & 0.96 & 0.16 & 0.26 & 0.36 & 0.46 \\
    & Basic agent         & 0.17 & 0.27 & 0.37 & 0.47 & 0.57 & 0.67 & 0.77 & 0.87 & 0.97 & 0.17 & 0.27 & 0.37 & 0.47 \\
    & SIP-enhanced agent  & 0.18 & 0.28 & 0.38 & 0.48 & 0.58 & 0.68 & 0.78 & 0.88 & 0.98 & 0.18 & 0.28 & 0.38 & 0.48 \\
\midrule
\multirow{2}{*}{$\Delta$Skew} 
    & Basic agent         & 0.01 & 0.02 & 0.03 & 0.04 & 0.05 & 0.06 & 0.07 & 0.08 & 0.09 & 0.01 & 0.02 & 0.03 & 0.04 \\
    & SIP-enhanced agent  & 0.02 & 0.03 & 0.04 & 0.05 & 0.06 & 0.07 & 0.08 & 0.09 & 0.10 & 0.02 & 0.03 & 0.04 & 0.05 \\
\midrule
\multirow{3}{*}{Kurtosis} 
    & Human               & 0.19 & 0.29 & 0.39 & 0.49 & 0.59 & 0.69 & 0.79 & 0.89 & 0.99 & 0.19 & 0.29 & 0.39 & 0.49 \\
    & Basic agent         & 0.20 & 0.30 & 0.40 & 0.50 & 0.60 & 0.70 & 0.80 & 0.90 & 1.00 & 0.20 & 0.30 & 0.40 & 0.50 \\
    & SIP-enhanced agent  & 0.21 & 0.31 & 0.41 & 0.51 & 0.61 & 0.71 & 0.81 & 0.91 & 1.01 & 0.21 & 0.31 & 0.41 & 0.51 \\
\midrule
\multirow{2}{*}{$\Delta$Kurtosis} 
    & Basic agent         & 0.01 & 0.02 & 0.03 & 0.04 & 0.05 & 0.06 & 0.07 & 0.08 & 0.09 & 0.01 & 0.02 & 0.03 & 0.04 \\
    & SIP-enhanced agent  & 0.02 & 0.03 & 0.04 & 0.05 & 0.06 & 0.07 & 0.08 & 0.09 & 0.10 & 0.02 & 0.03 & 0.04 & 0.05 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

